The Nuts and Bolts of Adopting Transformer in GANs

Transformer becomes prevalent in computer vision, especially for high-level vision tasks. However, adopting Transformer in the generative adversarial network (GAN) framework is still an open yet challenging problem. In this paper, we conduct a comprehensive empirical study to investigate the properties of Transformer in GAN for high-fidelity image synthesis. Our analysis highlights and reaffirms the importance of feature locality in image generation, although the merits of the locality are well known in the classification task. Perhaps more interestingly, we find the residual connections in self-attention layers harmful for learning Transformer-based discriminators and conditional generators. We carefully examine the influence and propose effective ways to mitigate the negative impacts. Our study leads to a new alternative design of Transformers in GAN, a convolutional neural network (CNN)-free generator termed as STrans-G, which achieves competitive results in both unconditional and conditional image generations. The Transformer-based discriminator, STrans-D, also significantly reduces its gap against the CNN-based discriminators.

==> sections/method_old.tex <==

\begin{figure}[t]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{12cm}{0cm}}
    \includegraphics[width=\linewidth]{figures/strans-g-arch.png}
    \end{center}
    % \vspace{-5pt}
    \caption{(a) an overview of our STrans-G, a CNN-free generator. (b) By modifying the original MLP residual block, we enable the Transformer blocks to serve as the `toRGB' module outputing an image tensor. }
    \label{fig:strans-g}
    
\end{figure}


\section{Methodology}

% In this section, we start by introducing the overall design of our LoTGAN in the case of unconditional generation. 
%
In this section, we first detail the architecture of a CNN-free \xxy{do we need to mention ``CNN-free'' so many times? Does not seem like a big deal to me...} generator with Swin Transformer \xxy{No need to mention Swin so early}.
%
Meanwhile, by analyzing the generated samples and the attention behavior, we reveal the local attention mechanism has a profound effect on image synthesis.
%
Finally, we discuss two specific problems in discriminators and conditional generators, respectively.




\subsection{STrans-G: Locality in Image Generation}

The self-attention module in Transformer blocks introduces the dynamical representative ability and brings the convenience of modeling long-range dependencies. 
%
However, heavy computational costs prevent its applications in high-resolution synthesis.
%
In addition, when generating high-frequency contents in high-resolution stages, modules should pay much attention to the local regions while attending to long-range features even harms the performance \xxy{I woundn't say like this}.
%
Thus, we propose a pure Transformer generator applying the local Transformer in high-resolution stages, termed STrans-G.

\textbf{Architecture.}
%
Figure~\ref{fig:strans-g} depicts the overall architecture of our STrans-G. 
%
In the unconditional generation, STrans-G adopts a latent code $z\sim \mathcal{N}(0, I)$ as the input, and then a linear projection layer projects it into a $(4\times 4 \times C)$ feature map.
%
Each spatial vector in this low-resolution feature is regarded as an input token to the following Transformer blocks.
%
To inject positional information~\cite{karras2021alias,xu2021positional}, we add a learnable positional encoding to the input tokens.
%
STrans-G gradually increases the resolution of the feature map through multiple Transformer blocks and upsampling operations. 
%
Except for the $64\times 64$ stage, we choose the bilinear upsampling operation in each stage. In the $64^2$ scale, we adopt pixel shuffle~\cite{shi2016real} operator to upsample features and reduce the channel dimension.
%
The last `toRGB' block generates image tensors with three channels.
%
As shown in Fig.~\ref{fig:strans-g}(b), we let the MLP module output a three-channel feature and add a linear layer on the skip connection to match the channel dimension.


%
In the first several stages, since the feature map has small spatial dimensions, we directly apply the standard Transformer block~\cite{dosovitskiy2020image} capturing the global structure.
%
However, the computational complexity of the standard self-attention module is $\mathcal{O}((HW)^2)$, where $H$ and $W$ are the height and width of the spatial feature map, respectively.
%
Such a quadratic complexity causes intractable computational and memory costs in dealing with high-resolution features, like $128\times 128$ features.
%
Recently, Swin Transformer~\cite{liu2021swin} introduces an effiecient local Transformer with linear computational complexity ($\mathcal{O}(HW)$).
%
Meanwhile, its shifted window attention effectively bridges local regions and keeps the ability to capture long-range dependencies. 
%
As shown in Fig.~\ref{fig:strans-g}(a), we switch to Swin Transformer when processing high-resolution features.
%
In general, we start adopting the Swin architecture from the $16 \times 16$ scale.
%


\begin{figure}[t]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{12cm}{0cm}}
    \includegraphics[width=\linewidth]{figures/locality.png}
    \end{center}
    \vspace{-5pt}
    \caption{(a) and (b) presents $64\times 64$ samples synthesized by Trans-G and STrans-G, respectively. In (c), we analyze the failure cases from Trans-G. The red arrow in (c) indicates the pixels obtaining the highest attention score in the last attention layer. In (d), we compare the averaged attention distance between the standard global attention and the swin attention. The statistics of the averaged attention distance is calculated in the last stage of the generator.}
    \label{fig:locality}
    
\end{figure}

\textbf{Importance of Locality. \xxy{put this part ahead of Architecture}} In addition to saving computational costs, another important motivation for adopting Swin architecture is to keep the locality of image data.
%
% In fact, locality-preserving operators are dominant in image processing, \eg,  the convolutional 
%
The locality~\cite{he2004locality} is a core assumption in designing operators for image processing, \eg, traditional Sobel operator~\cite{farid2004differentiation} and popular convolution layers~\cite{krizhevsky2012imagenet}.
%
In this part, we demonstrate the locality still has a profound effect on high-fidelity image generation.

We start by replacing all of Swin blocks with standard Transformer blocks in STrans-G. This new alternative is called Trans-G.
%
Chasing the best performance, we adopt the powerful discriminator proposed in StyleGAN2~\cite{karras2020analyzing} and differentiable data argmentation~\cite{karras2020training}. We train STrans-G and Trans-G in $64\times 64$ FFHQ dataset with the same training configuration.
%
In STrans-G, we set the window size to 4 by default.
%
More details can be found in Sec.~\ref{app:impl}.


Since the traditional attention module captures the global relationship, it is easier for Trans-G to learn long-range correspondence at each stage than our STrans-G.
%
Nevertheless, as shown in Fig.~\ref{fig:locality}(a), Trans-G always generates noisy artifacts and unreasonable structure leading to a worse FID~\cite{heusel2017gans}.
%
To reveal the cause for the degradation in Trans-G, we analyze the last high-resolution attention map which is most close to the final image feature.
%
The red arrows in Fig.~\ref{fig:locality}(c) point to the pixel with the highest attention score \wrt the query pixel.  
%
We observe that the self-attention module in Trans-G aggregates features from an unrelated distant region, \eg, the query pixel in the facial region attends to a background pixel. 


Furthermore, we compute the average distance between the query token position and the locations it attends to.
%
% The statistic of the attention distance from the self-attention modules in the highest scale is presented in Fig.~\ref{fig:locality}(d).
%
Figure \ref{fig:locality}(d) presents the distribution of the attention distance that is calculated from the self-attention modules on the highest scale.
%
Without any strict constraints, the global attention module always attends to pixels with a medium distance (10-20 pixels).
%
Meanwhile, it is unavoidable for Trans-G to attend to unreasonable distant pixels ($>$32 pixels) in the highest scale, which can easily result in the failure cases shown in Fig.~\ref{fig:locality}(c).
%
In contrast, with the window attention mechanism, STrans-G can efficiently compute local attention and guarantee the locality in high-resolution images.
%
Besides, in our experiments, we also find the locality in STrans-G can lead to an impressive performance in the challenging $256^2$ scale.
%

% Furthermore, Figure~\ref{fig:locality}(c) presents the statistics of the attentive in each attention head  

Aiming at reducing the quadratic computational complexity, several concurrent works start introducing local attention mechanisms into generators.
%
\cite{zhao2021improved, jiang2021transgan} propose the grid self-attention to calculate local attention in a $M\times M$ window. However, the grid attention in \cite{jiang2021transgan} lacks efficient connections between local regions.
%
The dilated attention in HiT\cite{zhao2021improved} remedies the loss of global attention, while its $\mathcal{O}((HW)^{1.5})$ computational complexity is still unaffordable for higher resolutions.
%
Because of this, HiT only applies Transformer blocks in low-resolution stages.
%
Different from them, an important motivation for STrans-G is following the locality assumption in the image domain.
%
In our experiments, we fairly compare different local attention mechanisms to verify the effectiveness of the Swin architecture.

\begin{figure}[t]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{12cm}{0cm}}
    \includegraphics[width=\linewidth]{figures/strans-d-arch.png}
    \end{center}
    \vspace{-5pt}
    \caption{(a) The overall architecture of STrans-D. In (b), we illustrate the detailed architecture of the Swin Transformer block with \bfit{skip-proj} in STrans-D. (c) presents the norm ratio between the shortcut and the main branch. `A' and `M' denotes the attention block and the MLP block, respectively. The number right after `A' and `M' indicates the layer index in the discriminator. The red vertical line in (c) represents a downsampling operation.}
    \label{fig:strans-d}
    
\end{figure}

\subsection{STrans-D: Degradation in Swin Transformer Discriminators}
\label{sec:strans-d}

\xxy{first summarize the methods; then explain them.}

With the StyleGAN2 discriminator, our CNN-free STrans-G shows impressive ability in the unconditional generation.
%
However, it is not trivial to design a Transformer-based discriminator which can enable STrans-G to converge efficiently and effectively.
%
When applying the original Swin Transformer as a discriminator, we meet unstable training procedures and inferior generation quality in $256\times 256$ FFHQ dataset.
%
In this section, we first detail how we improve the design of STrans-D step by step.
%
Then, we clarify the degradation problem in STrans-D and propose the subtle yet effective \bfit{skip-proj} module to remedy it.

\textbf{Architecture.}
%
Figure \ref{fig:strans-d}(a) illustrates the architecture of our STrans-D, a hybrid model composed of few convolutional layers and a Swin Transformer-based backbone.
%
We start by adopting a lite convolutional block to downsample the original input scale by $4\times$ times and project the image tensor to an arbitrary dimension (denoted as $C$).
%
Compared to the patch embedding module~\cite{dosovitskiy2020image} used in Transformer models, the convolution token extractor adopts overlapped patches keeping more detailed information.
%
By stacking Swin Transformer blocks with bilinear downsampling operation, the high-resolution input tokens are gradually downsampled to ($4\times 4 \times C$) feature.
%
Note that we discard the original patch merging module in \cite{liu2021swin} to avoid a large channel dimension. 
%
Containing a convolutional layer and several linear layers, the decision head outputs the final prediction.
%
% In fact, such a hybrid mix of convolutional blocks and Transformer backbone is proven to be more effective in high-level tasks in recent works~\cite{li2021localvit,xiao2021early}.
%
% To further strengthen the hybrid discriminator, we 


In the detailed implementation, we find the transformer blocks in such a hybrid discriminator must be trained with a small learning rate leading to slow and unsatisfactory convergence.
%
Inspired by \cite{karras2017progressive}, we adopt the equalized learning rate in all of the attention modules and feedforward modules in Swin Transformer blocks.
%
After that, we can set the whole discriminator with a large learning rate but offer a small learning rate scaler in the Transformer blocks (\xxy{more explanations here}).
%
This strategy significantly improves the convergence speed.
%
Additionally, we replace GeLU~\cite{hendrycks2016gaussian} with LeakyReLU~\cite{maas2013rectifier} as the default activation function.
%
Meanwhile, we add a nonlinear activation function at the end of the attention module and the MLP module in the Transformer blocks (\xxy{is this important?}). 

\textbf{Degradation in Discriminators.}
%
Despite that these efforts successfully improve the initial baseline, there still exists a significant gap between our STrans-D and StyleGAN2 discriminator.
%
To find the reason for the degradation, we plot the norm ratio~\cite{raghu2021vision} $||x_i|| / ||f(x_i)||$, where $x_i$ denotes the features from the shortcut and $f(x_i)$ indicates the transformation of $x_i$ from the residual branch.
%
The norm ratio can reflect the information flow in the network.
%
As shown in Fig.~\ref{fig:strans-d}(c), STrans-D performs an extremely high ratio in the $64\times 64$ stage, which indicates that the Transformer backbone neglects the high-resolution features and starts making differences from the $32\times 32$ resolution. 
%
Due to the lack of high-resolution features, STrans-D cannot offer accurate feedbacks for the detailed textures.
%
To avoid such unhealthy behavior, we apply a linear layer (Fig.~\ref{fig:strans-d}(b)) as a learnable scaler in the skip connection, termed as \bfit{skip-proj}. 
%
The comparison in Fig.~\ref{fig:strans-d}(c) proves that skip-proj prevents the escalation of the norm ratios in early stages.
%
Benefiting from the high-resolution features, STrans-D with \bfit{skip-proj} successfully reduces the gap from the StyleGAN2 discriminator. 

\begin{figure}[t]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{12cm}{0cm}}
    \includegraphics[width=0.9\linewidth]{figures/c-stransg-arch.png}
    \end{center}
    \vspace{-5pt}
    \caption{(a, b, c) show three alternative designs of adopting AdaNorm in a Transformer block. (d) presents the norm ratio between the shortcut and the residual branch. `A' and `M' denote the attention block and the MLP block, respectively. The number right after `A' and `M' indicates the layer index in the generator. The red vertical line in (d) represents an upsampling operation.}
    \label{fig:c-strans-g}
    
\end{figure}

\subsection{Conditional Generatorin with STrans-G}


%
% It is not trivial to achieve conditional generation with Transformer-based generators.
%
The direct shortcut in Transformer blocks still has a profound influence on the design of conditional generators. 
%
Typically, in convolutional GANs, we adopt AdaNorm~\cite{dumoulin2016learned,huang2017arbitrary,park2019SPADE} on the residual branch to inject category conditions:
%
\begin{equation}
    \label{eq:adanorm}
    \mathrm{AdaNorm}(x, y) = \gamma (y) \cdot \mathrm{Norm}(x) + \beta (y),
\end{equation}
%
where $x$ and $y$ are input features and conditions respectively.
%
$\mathrm{Norm}(\cdot)$ can be replaced with multiple normalization layers, \eg, Batch Normalization~\cite{ioffe2015batch}, and Instance Normalization~\cite{ulyanov2016instance}.
%
% To modulate the normalized features, $\gamma(\cdot)$ and $\beta(\cdot)$ project the condition vector $y$ to the variance tensor $\gamma(y)$ and the bias tensor $\beta(y)$.
%
$\gamma(\cdot)$ and $\beta(\cdot)$ modulate the normalized feature $\mathrm{Norm}(x)$ according to the conditional label $y$.
%
However, when replacing the original layer normalization~\cite{ba2016layer} layers in Transformer blocks with AdaLN (Fig.~\ref{fig:c-strans-g}(a)), we find the FID stops decreasing in the early stage.
%
Following the experience in STrans-D, we plot the norm ratio of this baseline configuration. 
%
As shown in Fig.~\ref{fig:c-strans-g}(d), there exist several blocks performing a large norm ratio. This indicates that some AdaLN layers in the residual branch cannot contribute to the intermediate features.
%
Thus, we rethink the way of adopting AdaNorm and propose a general strategy for applying AdaNorm in Transformer blocks, termed as \bfit{AdaNorm-T}.

%
To guarantee the conditional information is injected into the output features, a straightforward way is applying the AdaNorm in the trunk, as shown in config-b in Fig.~\ref{fig:c-strans-g}.
%
In this case, the features from the shortcut and the MLP branch both contain class information. 
%
In fact, the AdaNorm layers in the trunk unintentionally bring the norm ratio below the baseline config-a in Fig.~\ref{fig:c-strans-g}(a).


However, we observe that only applying AdaNorm in the truck causes undesirable mode collapse in several training cases.
%
Since the mode collapse reflects a failure in modeling global structure, we focus on the early attention blocks which compute global attention.
%
As shown in Fig.~\ref{fig:c-strans-g}(c), after adopting another AdaNorm at the end of the attention block, we find the mode collapse disappears in the early stage.
%
The norm ratio in Fig.~\ref{fig:c-strans-g}(d) shows that the AdaNorm at the end of the attention module leads to an extremely high ratio in the second and third attention blocks.
%
This indicates that $\gamma(y)$ and $\beta(y)$ in Eq.~(\ref{eq:adanorm}) can serve as a learnable gating helping networks to skip collapsed features.
%

In summary, Fig.~\ref{fig:c-strans-g}(c) illustrates our strategy for adopting AdaNorm in Transformer blocks. Note that the AdaNorm after the attention modules is only adopted in the global attention blocks. Because, we find applying it in Swin attention blocks cannot further improve the generation quality. We verify the effectiveness of \bfit{AdaNorm-T} in CIFAR10 with \bfit{AdaIN-T} and \textsc{ImageNet} with \bfit{AdaBN-T}.
%

% To our knowledge, this study is the first one to perform conditional generation with a pure Transformer generator.

==> sections/statement.tex <==
% \vspace{-5pt}
\section{Ethics and Reproducibility Statement}
\vspace{-5pt}
%
\noindent\textbf{Ethics Statement.}
%
This work improves the image generation quality, which can facilitate the movie industry and virtual reality.
%
However, there could be potentially inappropriate applications of this technique, lying in various forms of disinformation, \eg, synthesizing fake portraits in different scenes~\cite{perov2020deepfacelab}. Our work may unintentionally make these applications more convincing or deceiving.
%
Viable solutions to prevent misusage and negative effects include developing robust methods to detect fake content generated by deep models~\cite{tolosana2020deepfakes} and adopting model watermarking~\cite{yu2020artificial}.


\noindent\textbf{Reproducibility Statement.}
%
We have provided the necessary implementation details in Sec.~\ref{sec:method}, Sec.~\ref{sec:exp}, and Appendix \ref{app:impl}. In addition, we also include more results with different settings of STransGAN in Appendix \ref{app:impl}. Our training pipeline follows standard training configurations in current literature and does not include extra tricks. The models and codes will be publicly available.
